Higher-order Weierstrass weights of branch points on superelliptic curves

In this paper we consider the problem of calculating the higher-order Weierstrass weight of the branch points of a superelliptic curve $C$. For any $q>1$, we give an exact formula for the $q$-weight of an affine branch point. We also find a formula for the $q$-weight of a point at infinity in the case where $n$ and $d$ are relatively prime. With these formulas, for any fixed $n$, we obtain an asymptotic formula for the ratio of the $q$-weight of the branch points, denoted $BW_q$, to the total $q$-weight of points on the curve: \[ \liminf_{d\to\infty}\frac{BW_q}{g(g-1)^2(2q-1)^2}\geq \frac{n+1}{3(n-1)^2(2q-1)^2},\] with equality when the limit is taken such that $\gcd(n,d)=1$.

==> macro_g_3.tex <==
\usepackage{ amsmath,amssymb,amsbsy,amsfonts, latexsym,amsopn,amstext, amsxtra,euscript,amscd, hyperref}
\usepackage{graphicx}
%\usepackage{cite}
\usepackage{cite}

\usepackage{amsrefs}

\usepackage{url}

%\usepackage{xy} \input xy \xyoption{all}
%\usepackage{amscd, epic, amssymb}
%\usepackage{latexsym, color}
%\usepackage{amscd, psfig, epsfig}

\newcommand\myurl[1]{\url{#1}}

\BibSpec{webpage}{%
  +{}{\PrintAuthors} {author}
  +{,}{ \textit} {title}
  +{}{ \parenthesize} {date}
  +{,}{ \myurl} {myurl}
  +{,}{ } {note}
  +{.}{ } {transition}
}




\usepackage{xy} 
\input xy \xyoption{all}

%\setlength{\textwidth}{6.9in}
%\setlength{\textheight}{8.8in}
%\setlength{\topmargin}{-.65in}
%\setlength{\oddsidemargin}{-.5cm}
%\setlength{\evensidemargin}{-.7cm}
%\setlength{\columnsep}{2.0pc}



\def\ss{\mathfrak s}
%*************************definitions**************************



\newtheorem{thm}{Theorem}
\newtheorem{prop}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{rem}{Remark}
\newtheorem{cor}{Corollary}
\newtheorem{exa}{Example}

%\theoremstyle{defn}
\newtheorem{defn}{Definition}
\newtheorem{conj}{Conjecture}
\newtheorem{prob}{Problem}

%   \mathbb

\def\Z{\mathbb Z}
\def\Q{\mathbb Q}
\def\C{\mathbb C}
\def\P{\mathbb P^1 (k)}
\def\Q{{\mathbb Q}}
\def\Z{{\mathbb Z}}
\def\C{{\mathbb C}}
%\def\xs{{\mathbb o}}
%\def\xs{{\Bbb o}}
\def\bP{{\mathbb P}}

% mathcal 

\def\L{\mathcal L}
\def\H{\mathcal H}
\def\M{\mathcal M}
\def\X{\mathcal X}
\def\S{\mathcal S}

\def\cB{\mathcal B}
\def\cA{\mathcal A}
\def\cR{\mathcal R}
\def\N{\mathcal N}



% mathfrak 

\def\p{\mathfrak p}
\def\u{\mathfrak u}
\def\v{\mathfrak v}
\def\ss{\mathfrak s}
\def\u{\mathfrak u}
\def\u{\mathfrak s}
\def\p{\mathfrak p}
\def\s{\mathfrak s}
\def\v{\mathfrak v}


% others



\def\Pic{\mbox{Pic }}
\def\Jac{\mbox{Jac }}



%\def\Aut{\mbox{ Aut}}
%\def\bAut{\overline {\mathrm{Aut}}}
\def\D{\Delta}


\def\emb{\hookrightarrow}

\def\l{\lambda}
%\def\s{\sigma}
\def\a{\alpha}
\def\e{\varepsilon}
\def\b{\beta}

\def\w{\widetilde}
\def\t{\tau}
\def\<{\langle}
\def\>{\rangle}
\def\zz{\zeta}
\def\z{\omega} 



\def\iso{{\, \cong\, }}
\def\ch{\mbox{char }}


\def\bG{\bar G}
\def\G{G}

%%%%%%% ketu 




\def\bG{{\bar G}}
\def\bg{{\bar g}}
\def\g{{g}}
\def\bZ{{\mathbb Z}}

\def\diag{\mbox{diag }}

\def\sem{{\rtimes}}
 
%\def\ss{\mathfrak s}


\def\Z{\mathbb Z}
\def\R{\mathbb R}
\def\Q{\mathbb Q}
\def\bC{\mathbb C}
\def\C{\mathbb C}


\def\C{\mathcal C}
\def\H{\mathcal H}
\def\M{\mathcal M}

\def\w{\widetilde}
\def\l{\lambda}
\def\a{\alpha}
\def\b{\beta}
\def\p{\mathfrak p}
%\def\iso{\equiv}



\def\Z{\mathbb Z}
\def\Q{\mathbb Q}
\def\C{\mathbb C}
\def\L{\mathcal L}
\def\H{\mathcal H}
\def\M{\mathcal M}
\def\l{\lambda}
\def\s{\sigma}
\def\a{\alpha}
\def\p{\mathfrak p}
\def\u{\mathfrak u}
\def\v{\mathfrak v}
%\def\iso{{\, \cong\, }}
\def\<{\langle}
\def\>{\rangle}
\def\X{\mathcal X}
%\def\Aut{\mathrm{Aut}}
%\def\bAut{\overline {\mathrm{Aut}}}
\def\emb{\hookrightarrow}

\def\D{\Delta}
%\def\ss{\mathfrak s}

\def\u{\mathfrak u}
\def\L{\mathcal L}

%\def\T{\theta}
%\def\Aut{\rm Aut}

\def\S{\mathcal S}


\def\Y{\mathcal Y}
\def\A{\mathcal A}
\def\B{\mathcal B}


\def\P{\mathbb P^1 (k)}
\def\Q{{\mathbb Q}}
\def\Z{{\mathbb Z}}
\def\C{{\mathbb C}}
\def\M{{\mathcal M}}
\def\H{\mathcal H}
\def\L{\mathcal L}

\def\J{\mbox{Jac }}
\def\O{\Omega}
\def\T{\theta}

\def\Aut{\mbox{Aut }}
\def\bAut{\overline {\mathrm{Aut}}}

\def\Pic{\mbox{Pic }}
\def\Jac{\mbox{Jac }}

%\def\iso{\equiv}

\def\embd{\hookrightarrow}

%\newcommand\G{\bar G}
\def\D{\Delta}
\def\e{\varepsilon}
\def\u{\mathfrak s}

\def\g{\gamma}
\def\bG{\bar G}
\def\t{\tau}
\def\d{{\delta }}
\def\a{{\alpha }}
\def\b{{\beta }}
\def\c{\textbf{c}}

\def\bC{\mathfrak \si}
%\def\cong{\equiv}

\def\th{\theta}
\def\<{\langle}
\def\>{\rangle}

\def\diag{\mbox{diag }}
%\def\mychar{\mbox{char }} 
\def\sem{{\rtimes}}

%\def\s{{\sigma }}
\def\s{\mathfrak s}


\def\v{\mathfrak v}

\def\r{\gamma}
%\def\si{\si}

%\def\ss{$\mathfrak s$}

\def\p{\mathfrak p}

\newcommand{\cH}{\mathcal H}
%\newcommand{\mychar}{\mbox{char }}

\newcommand\F{\mathbb F}

\def\emb{\hookrightarrow }
\def\tr{{\mbox tr }}

\def\U{\mathcal U}

\def\normal{\triangleleft}


\def\xs{{\mathbb o}}
\def\xs{{\Bbb o}}
\def\zz{\zeta}

\def\z{\omega} 

\def\k{\bar k}

%\def\e{\epsilon}


%\def\A{\mbox{Aut}} \def\AA{\overline{\A}}

%\def\P{P} \def\a{p}

\def\V{V_4}





